Scalable Measurement Error Mitigation via Iterative Bayesian Unfolding

Measurement error mitigation (MEM) techniques are postprocessing strategies to counteract systematic read-out errors on quantum computers (QC). Currently used MEM strategies face a tradeoff: methods that scale well with the number of qubits return negative probabilities, while those that guarantee a valid probability distribution are not scalable. Here, we present a scheme that addresses both of these issues. In particular, we present a scalable implementation of iterative Bayesian unfolding, a standard mitigation technique used in high-energy physics experiments. We demonstrate our method by mitigating QC data from experimental preparation of Greenberger-Horne-Zeilinger (GHZ) states up to 127 qubits and implementation of the Bernstein-Vazirani algorithm on up to 26 qubits.

==> main_old.tex <==
% \documentclass[american,aps,pra,reprint,floatfix,nofootinbib,superscriptaddress]{revtex4-2}
% \usepackage[unicode=true,pdfusetitle, bookmarks=true,bookmarksnumbered=false,bookmarksopen=false, breaklinks=false,pdfborder={0 0 0},backref=false,colorlinks=false]{hyperref}
% \hypersetup{colorlinks,linkcolor=blue,citecolor=red,urlcolor=cyan}
% \usepackage{graphics,epstopdf,amsthm,amsmath,amssymb,mathptmx,colortbl,color,bm,framed,mathrsfs}
% \usepackage{comment}
% \usepackage{csquotes}
% \usepackage[T1]{fontenc}
% \usepackage[up]{subfigure}
% \usepackage[braket, qm]{qcircuit}
% \usepackage{physics}
% \usepackage{commath}
% \usepackage{mathtools}
% \usepackage{float}
% \usepackage{appendix}
% \usepackage{amsthm}
% \usepackage[linesnumbered, ruled,vlined]{algorithm2e}
% \usepackage{dsfont}
% \usepackage{nicefrac}
% \usepackage[capitalise]{cleveref}
% \bibliographystyle{apsrev4-2}
% \DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
% \makeatother

% %color commands
% \newcommand{\red}{\textcolor{red}}
% \newcommand{\blue}{\textcolor{blue}}

% %figures side-by-side
% \usepackage[demo]{graphicx}
% %\usepackage{caption}
% %\usepackage{subcaption}
% \usepackage{centernot}

% %package to strikeout text
% \usepackage[normalem]{ulem}
% %\sout{Hello World}

% \usepackage{csquotes}

% \usepackage{xcolor}
% \newcommand{\bbk}[1]{\textcolor{red}{B: #1}}


% \begin{document}


% \title{Scalable unfolding for measurement error mitigation}


% \author{Bibek Pokharel}
% \email{pokharel@usc.edu}
% \affiliation{Department of Physics and Astronomy, University of Southern California, Los Angeles, CA, 90089, USA}
% \affiliation{Center for Quantum Information Science \& Technology, University of Southern California, Los Angeles, CA 90089, USA}

% \author{Siddarth Srinivasan}
% \affiliation{Department of Computer Science and Engineering, University of Washington}

% % \author{Daniel A. Lidar}
% % \email{lidar@usc.edu}

% % \affiliation{Department of Physics and Astronomy, University of Southern California, Los Angeles, CA, 90089, USA}
% % \affiliation{Center for Quantum Information Science \& Technology, University of Southern California, Los Angeles, CA 90089, USA}
% % \affiliation{Department of Electrical Engineering, University of Southern California, Los Angeles, CA, 90089, USA}
% % \affiliation{Department of Chemistry, University of Southern California, Los Angeles, CA, 90089, USA}

% \author{Byron Boots}
% \affiliation{Department of Computer Science and Engineering, University of Washington}


% \date{\today}

% \begin{abstract}
% Measurement errors are one of programmable quantum computers' most significant noise sources. Measurement error mitigation (MEM) techniques are postprocessing strategies to counteract systematic measurement errors. The most common MEM methods model errors as a linear stochastic map, also called the response or confusion matrix, and aim to invert its effect. This inversion strategy has two issues: firstly, the response matrix is not bistochastic, and so it returns quasiprobabilities, and secondly, it scales exponentially with the number of qubits. Building on previous MEM strategies, we demonstrate a method that does not scale exponentially with the number of qubits, avoids using quasiprobabilities and performs better than its predecessors. In particular, our strategy enforces a k-locality and a precision threshold to the data, and then performs iterative Bayesian unfolding initialized with physically motivated priors. We demonstrate our method with experimental preparation of 82-qubit GHZ state and implementation of 27-qubit Bernstein-Vazirani algorithm. . 
% \end{abstract}
% \maketitle


% \section{Introduction}


% Measurement errors are a significant source of errors for quantum devices. Quantum readout error mitigation (QREM) techniques are a collection of classical post-processing techniques that aim to address these measurement errors at the software level. Most QREM methods assume that measurement errors are systematic, linear, and time-independent. These simplifying assumptions are worth verifying before applying QREM to any QC. Fortunately,  previous work \cite{maciejewskiMitigationReadoutNoise2020} has established that these simplifying assumptions are mostly accurate for IBM Quantum Experience (IBMQE) superconducting devices, provided the readout calibration data is up to date.

% Systematic measurement errors are quantified using a response matrix $R$, which is obtained after performing quantum detector tomography (QDT) \cite{maciejewskiMitigationReadoutNoise2020}. The entries of the response matrix are simply conditional probabilities -- the probability of measuring a certain bitstring $b_1$ given that computational basis element $| b_2 \rangle$ was prepared. Both acquiring $R$ and implementing QREM face two main challenges: \emph{scaling} and \emph{non-negativity}. First, $R$ is a $2^n \times 2^n$ matrix for a $n$-qubit system and in general requires $2^n$ calibration experiments. In other words, QDT requires exponentially many experiments. Second, while the response matrix $R$ is stochastic, its inverse is not. As most QREM methods rely on applying $R^{-1}$, this leads to a `negative probability' issue -- the distributions obtained after measurement error mitigation are \emph{quasiprobabilities}, i.e., the elements of this quasiprobability distribution sum to unity but can be negative. Since the introduction of QREM to the quantum computing literature, several attempts have addressed the scalability and negativity issues.

% The scalability issue has two aspects: QDT requires exponentially many calibration experiments in the number of qubits, and QREM requires inversion and matrix multiplication with a large matrix that also grows exponentially in the number of qubits. Assuming $k$-locality for $R$ \cite{bravyiMitigatingMeasurementErrors2021, maciejewskiMitigationReadoutNoise2020} (i.e., only $k$ qubits have a measurement cross-talk) allows $R$ to be represented as $\nicefrac{n}{k}$ different $2^k \times 2^k$ matrices. This assumption has been verified in Refs~\cite{nationScalableMitigationMeasurement2021, maciejewskiMitigationReadoutNoise2020} and presents the first step in addressing the scalability issue. The unmitigated probability distributions are already sparse as the experiments required to construct these distributions are only performed for $s$ shots, and in practice $s$ will not scale exponentially with qubit size due to time and computational constraints. Ref~\cite{nationScalableMitigationMeasurement2021} relied on this sparsity to further speedup QREM. In particular, only the matrix elements of $R$ that had bitstrings close to the observed ones (measured using Hamming distance) could be considered, while others were ignored. This subspace reduction of $R$ suggested that a user could perform QDT after and with the knowledge of the unmitigated experimental results. In other words,  the order of QDT and the experiment was flipped. Similarly, Ref.~\cite{mooneyGenerationVerification27qubit2021} suggested placing a precision threshold on $R$ and QREM, such that any probabilities below $\nicefrac{1}{(10\times s)}$ are ignored. These approaches to scaling QREM have shown to be quite effective. In particular, Ref.~\cite{mooneyGenerationVerification27qubit2021, nationScalableMitigationMeasurement2021, yangEfficientQuantumReadout2022} have demonstrated GHZ state preparation on 27, 42 and 65-qubits respectively. QREM plays a crucial part in each of these demonstrations; without QREM, the success metrics are significantly lower.

% As for the negativity issues, numerous methods have been proposed but no clear consensus has emerged. As all the scalable methods listed above aim to invert and apply $R^{-1}$, the non-stochasticity of $R^{-1}$ necessarily leads to quasiprobabilities. A common strategy is to use constrained least-squares optimization to find the probability distribution closest mitigated quasiprobability distribution. Alternatively, the negative terms can be canceled systematically, as detailed in Ref.~\cite{smolinEfficientMethodComputing2012}. Ref.~\cite{nachmanUnfoldingQuantumComputer2020}  highlighted that error-prone detectors are standard across experimental fields, and unfolding techniques that are used in high-energy physics experiments can be used to mitigate readout errors on quantum devices. In particular, Ref.~\cite{nachmanUnfoldingQuantumComputer2020} showed that iterative Bayesian unfolding (IBU)~\cite{dagostiniMultidimensionalUnfoldingMethod1995} could be used to mitigate readout errors without compromising on non-negativity. At the same time, IBU requires iterative matrix multiplications with $R$ and therefore presents a greater challenge to scalability compared to response matrix inversion. In this work, we show that under reasonable and common assumptions about measurement crosstalk and precision, IBU can be implemented scalably and without producing negative probabilities in the error-mitigated distribution. Moreover, our implementation performs well across a variety of metrics. 

% % We show that IBU is EM.
% While IBU calls for iterative applications of Bayes' theorem and starts with an initial guess of the mitigated distribution sometimes called a `prior', it is not actually computing a posterior and therefore not a Bayesian method. In fact, it is more appropriate to call it iterative expectation maximization unfolding~\cite{volobouevExpectationMaximizationUnfoldingSmoothing2015} as it converges to the maximum likelihood estimate~\cite{sheppMaximumLikelihoodReconstruction1982} for large number of iterations. For pedagogical purposes, we provide a derivation of IBU as expectation maximization. 


% % Unlike \citep{nation2021scalable}, our method does not produce negative probabilities.

% % Unlike former IBU implementations, our method is scalable since we use the subspace reduction trick from \citep{nation2021scalable}.

% \begin{figure}
%  \begin{displaymath}
% \large
% \Qcircuit @C=1em @R=0.9em @!R {
%  &  \mbox{Quantum Detector Tomography} &   \\
% \lstick{| 0 \rangle}  & \multigate{4}{\text{State Preparation}} & \meter  \\
% \lstick{| 0 \rangle}  & \ghost{\text{State Preparation}}        & \meter  \\
%                       & \ghost{\text{State Preparation}} 	& \vdots  \\
% \lstick{| 0 \rangle}  & \ghost{\text{State Preparation}} 	& \meter  \\
% \lstick{| 0 \rangle}  & \ghost{\text{State Preparation}} 	& \meter  
% }
%     \end{displaymath}


%     \begin{displaymath}
% \large
% \Qcircuit @C=1em @R=0.9em @!R {
%  & & & \text{Error-mitigated experiment} &  &   \\
% \lstick{| 0 \rangle}  & \multigate{4}{\text{U}} & \meter  & \cw	   & \cw & \cw &  & & \cw		\\
% \lstick{| 0 \rangle}  & \ghost{\text{U}}        & \meter  & \cw    & \cw & \cw & &  & \cw      		\\
%                       & \ghost{\text{U}} 	&   	  & \vdots & 	 & & \push{\text{MEM}} & & \cw		\\
% \lstick{| 0 \rangle}  & \ghost{\text{U}} 	& \meter  & \cw    & \cw & \cw & &  & \cw       		\\
% \lstick{| 0 \rangle}  & \ghost{\text{U}} 	& \meter  & \cw    & \cw & \cw & &  & \cw \gategroup{2}{6}{6}{8}{1.2em}{--} \\}
%     \end{displaymath}
%     \caption{Measurement error mitigation schemes require two separate steps. First, quantum detector tomography (QDT) must be performed to acquire the response matrix (see top). If no assumptions are made about measurement cross-talk then $2^n$ computational basis states must be prepared during QDT. If we assume that there is k-locality in the measurement crosstalk then k-qubits can be grouped together and the corresponding response matrices can be tensored accordingly. Once the response matrix has been learnt, MEM can be applied to all future experiments. In particular, (see bottom) after applying a unitary $U$, the classical measurement data is fed into a MEM scheme to produce a new probability distribution. If the measurement calibration is reliable over time, then QDT can be performed sparingly.  }
%     \label{fig:mem-setup}
% \end{figure}


% % We also vectorize our IBU implementation, and put things on the GPU and use other parallelism available in JAX, maybe run things on colab.

% \section{Iterative Bayesian Unfolding as Expectation-Maximization}

% Here we give a simple derivation showing that iterative Bayesian unfolding for QREM is an instantiation of the well-known \emph{Expectation-Maximization} (EM) algorithm in machine learning with multinomial distributions. EM is a standard maximum-likelihood approach to estimating the parameters of latent variable models where optimizing the likelihood analytically and directly is not possible. The EM algorithm iterates between an \emph{E-step} which estimates a conditional expected likelihood under a given choice of model parameters, and an \emph{M-step} which updates the model parameters to maximizes the aforementioned conditional likelihood. EM maximizes a lower bound of the likelihood at every iteration, and thus every parameter update increases the likelihood. The method is guaranteed to converge to a local maximum. Although EM is a well-studied problem in machine learning, its connection to IBU may not be familiar to a quantum computing audience. Thus, we present a derivation of IBU as standard EM for mixture models and emphasize the theoretical justification for IBU.


% \paragraph{Setup}
% Assume all measurements are made in a fixed basis. Let $Z$ be the discrete random variable denoting $N$-length bitstrings with $P(Z)$ be the distribution over bitstrings prepared by the quantum computer. Due to measurement error, the distribution over bitstrings that are actually measured is different, and we denote this with random variable $X$ with distribution $P(X)$. Suppose we collect a dataset of $D$ measured bitstrings ${\bf X} = \{X_1, \ldots, X_D\}$ sampled IID from $P(X)$, and that we have access to the error model $P(X|Z)$ (i.e., the response matrix $R$ through QDT). Our goal is to estimate $P_\theta(Z)$, where $\theta$ is $2^N$-dimensional vector summing to 1 that parameterizes the true multinomial distribution over bitstrings prepared by our quantum computer.

% \paragraph{Likelihood}
% To see why EM is needed, observe that the likelihood of observing our data given a choice of parameter $\theta$ can be written as:
% \begin{equation}
%         P( {\bf X}; \theta) = \prod_{i=1}^D \sum_{j=1}^{2^N} P(X_i | Z_j) P_\theta(Z_j)
% \end{equation}
% Although we can take the log likelihood to eliminate the product, we are left an irreducible sum inside the log that makes it difficult to analytically solve for the optimal paramters:
% \begin{equation}\label{eq:loglik}
%         \ell(\theta; {\bf X}) =  \log P( {\bf X}; \theta) = \sum_{i=1}^D \log \left(\sum_{j=1}^{2^N} P(X_i | Z_j) P_\theta(Z_j) \right)
% \end{equation}

% EM is designed to get around this issue by instead maximizing a lower bound of the log-likelihood $\ell(\theta; {\bf X})$.

% \paragraph{Expectation-Maximization} We begin by observing that if we knew the parameters $\theta$, we could easily compute the joint probability of any observed bitstring and the `true' bitstring (i.e., the bitstring that would have been measured except for measurement error) as $P(X_i, Z_j; \theta) = P(X_i|Z_j)P_\theta(Z_j)$. At the same time, if we knew the joint probability $P(X_i, Z_j; \theta)$ of any observed bitstring and any given latent bitstring, we would be able to invert the previous equation to infer parameters $\theta$. EM turns this logic into an iterative algorithm that alternates between computing the conditional expected joint log likelihood of observed and latent bitstrings given parameters $\theta_t$ and finding the parameter $\theta_{t+1}$ that maximizes this conditional expected log likelihood. By Jensen's inequality, we can manipulate Eq \ref{eq:loglik} as:
% \begin{equation}\small \label{eq:bound}
% \begin{split}
%     \ell(\theta; {\bf X}) &= \sum_{i=1}^D \log \left(\sum_{j=1}^{2^N} P(X_i | Z_j) P_\theta(Z_j) \right) \\
%     &= \sum_{i=1}^D \log \left(\sum_{j=1}^{2^N} P(X_i | Z_j) P_\theta(Z_j) \frac{P_{\theta_t}(Z_j|X_i)}{P_{\theta_t}(Z_j|X_i)} \right) \\
%     &= \sum_{i=1}^D \log \left(\sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \frac{P(X_i | Z_j) P_\theta(Z_j)}{P_{\theta_t}(Z_j|X_i)} \right) \\
%     &\geq \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log \left( \frac{P(X_i, Z_j; \theta)}{P_{\theta_t}(Z_j|X_i)} \right) 
%     \end{split}
% \end{equation}

% Let $\hat{\ell}(\theta | \theta_t; {\bf X}) := \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log \left( \frac{P(X_i, Z_j; \theta)}{P_{\theta_t}(Z_j|X_i)} \right)$ be the lower bound of the log-likelihood $\ell(\theta; {\bf X})$. We can maximize this lower bound locally by updating the parameter at a given time-step $\theta_t$ as follows:

% \begin{equation}
%     \begin{split}
%         \theta_{t+1} &= \underset{\theta}{\text{arg max }}\sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log \left( \frac{P(X_i, Z_j; \theta)}{P_{\theta_t}(Z_j|X_i)} \right)  \\
%         &= \underset{\theta}{\text{arg max }} \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log P(X_i, Z_j; \theta) 
%     \end{split}
% \end{equation}

% Define $\ell(\theta | \theta_t; {\bf X}) := \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log P(X_i, Z_j; \theta) $, and note that maximizing $\hat{\ell}(\theta | \theta_t; {\bf X})$ is equivalent to maximizing $\ell(\theta | \theta_t; {\bf X})$.  EM consists of an \emph{E}-step which involves computing $\ell(\theta | \theta_t; {\bf X})$ and an \emph{M}-step which involves computing ${\text{arg max}_\theta} \ell(\theta | \theta_t; {\bf X})$. For computational reasons, we will combine these into a single step for updating parameter $\theta_t$ to $\theta_{t+1}$. To locally maximize $\ell(\theta | \theta_t; {\bf X})$, we can take the derivative (using the Lagrange multiplier $\lambda$ to enforce the normalization constraint that $\sum_j \theta_j = 1$).

% \begin{equation} \small
%     \begin{split}
%         &\phantom{=} \frac{\partial }{ \partial \theta_k} \left( \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log P(X_i, Z_j; \theta)  + \lambda \left(1 - \sum_{j=1}^{2^N} \theta_j \right) \right)\\
%         &= \frac{\partial }{ \partial \theta_k} \left( \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log P_\theta(Z_j) + \lambda \left(1 - \sum_{j=1}^{2^N} \theta_j \right) \right) \\
%         &= \frac{\partial }{ \partial \theta_k} \left( \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log \theta_j + \lambda \left(1 - \sum_{j=1}^{2^N} \theta_j \right)  \right) \\
%         &= \left(\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)\frac1{\theta_k} - \lambda
%     \end{split}
% \end{equation}

% Setting this to zero, we get $\theta_k = \frac1{\lambda}\left(\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)$, and by the requirement that $\sum_k \theta_k = 1 \Rightarrow \sum_k \frac1{\lambda}\left(\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right) = 1 \Rightarrow \lambda =  \sum_{i=1}^D \sum_k P_{\theta_t}(Z_k|X_i) = \sum_{i=1}^D 1 = D$. Substituting this back in, we get our update rule for each element $\theta_k$ of $\theta$ that locally maximizes the log-likelihood given an initial guess $\theta_t$:

% \begin{equation}
%     \left(\theta_{t+1}\right)_k = \frac1D \sum_{i=1}^D P_{\theta_t}(Z_k|X_i)
% \end{equation}

% Note that by Bayes' rule, we have $ P_{\theta_t}(Z_k|X_i) = \frac{P(X_i | Z_k) P_{\theta_t}(Z_k)}{\sum_i P(X_i | Z_k) P_{\theta_t}(Z_k)}$. Additionally, instead of summing over every bitstring in the dataset, we can re-write the sum as over all possible bitstrings using bitstring counts $n(X_i)$. Doing so, we end up with the IBU update rule:

% \begin{equation}\label{eq:ibu}
%     \left(\theta_{t+1}\right)_k = \sum_{i=1}^{2^N} \frac{n(X_i)}D  \cdot \frac{P(X_i | Z_k) P_{\theta_t}(Z_k)}{\sum_i P(X_i | Z_k) P_{\theta_t}(Z_k)}
% \end{equation}

% This is also the standard EM update rule for discrete mixture models in the machine learning literature. The only difference is that we treat the noise model $P(X_i|Z_j)$ as fixed, but the ML literature typically treats this as also as a parameter that can be updated through EM.

% \paragraph{Convergence of EM}  From Equation \ref{eq:bound}, we know that $\hat{\ell}(\theta | \theta_t; {\bf X})$ lower bounds the log-likelihood of the data ${\ell}(\theta; {\bf X})$, i.e., that ${\ell}(\theta; {\bf X}) \geq \hat{\ell}(\theta | \theta_t; {\bf X})$. We can further show that these two functions coincide at the current choice of parameter values $\theta = \theta_t$:
% \begin{equation}
% \begin{split}
%     \hat{\ell}(\theta_t | \theta_t; {\bf X}) &= \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log \left( \frac{P(X_i, Z_j; \theta_t)}{P_{\theta_t}(Z_j|X_i)} \right) \\
%     &= \sum_{i=1}^D \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i) \log P(X_i; \theta_t) \\
%     &= \sum_{i=1}^D \log P(X_i; \theta_t) \sum_{j=1}^{2^N} P_{\theta_t}(Z_j|X_i)  \\
%     &= \sum_{i=1}^D \log P(X_i; \theta_t) \cdot 1 \\
%     &= \ell(\theta_t; {\bf X})
% \end{split}
% \end{equation}

% Together, these facts imply that any choice of $\theta_{t+1}$ which improves $\hat{\ell}(\theta_{t+1} | \theta_t; {\bf X})$ from the current estimate $\hat{\ell}(\theta_t | \theta_t; {\bf X})$ must also improve the log-likelihood, i.e., $\hat{\ell}(\theta_{t+1} | \theta_t; {\bf X}) > \hat{\ell}(\theta_t | \theta_t; {\bf X}) \Rightarrow \ell(\theta_{t+1}; {\bf X}) > \ell(\theta_t; {\bf X})$ since $\ell(\theta_{t+1}; {\bf X})  \geq \hat{\ell}(\theta_{t+1} | \theta_t; {\bf X}) > \hat{\ell}(\theta_t | \theta_t; {\bf X}) = \ell(\theta_t; {\bf X}) $. Since EM updates $\theta_t$ to maximize $ \hat{\ell}(\theta | \theta_t; {\bf X})$ locally, the log-likelihood $\ell(\theta_t; {\bf X})$ increases at every iteration. Indeed, the log-likelihood increases by at least the amount $\hat{\ell}(\theta_{t+1} | \theta_t; {\bf X}) - \hat{\ell}(\theta_t | \theta_t; {\bf X})$. The algorithm iterates until it reaches a stationary point of $\hat{\ell}(\theta | \theta_t; {\bf X})$. Since $\hat{\ell}(\theta | \theta_t; {\bf X})$ is tangent to the log likelihood $\ell(\theta; {\bf X})$ at $\theta = \theta_t$ \citep{bishop2006pattern}, the termination also coincides with a stationary point of the log-likelihood. Thus, EM converges to a local stationary point of the log likelihood.


% % \section{Quantum IBU}

% % Thus far, we assumed that the measurements are made in a fixed basis. However, since we are dealing with quantum systems we may wish to infer the full \emph{density matrix} prepared by the quantum computer, with noisy measurements made in different bases. Essentially, this is the problem of measurement error mitigation for quantum state tomography under the assumption that the measurement error model  $\mathcal{E}(\cdot)$ is known.

% % \subsection{Notation}

% % Formally, let $\rho_Z$ be the quantum state prepared by the quantum computer. Due to measurement error $\mathcal{E}$ (assumed known), the noisy quantum state we can make measurements on is $\rho_X = \mathcal{E}(\rho_Z)$. Our goal is to estimate the original density matrix $\rho_Z^{\theta}$ through measurements on $\rho_X$, where $\theta$ parameterizes the density matrix we wish to estimate. Assume we collect data by making projective measurements $\Pi_i$ on $\rho_X$ and obtain dataset ${\bf X} = \{\Pi_1, \ldots, \Pi_D\}$.

% % \subsection{Likelihood}

% % The log likelihood of our measurements under choice of parameter $\theta$:

% % \begin{equation}
% %     \log P({\bf X}; \theta) = \sum_{i=1}^D \log \text{tr}\left( \Pi_i \mathcal{E}(\rho_Z^\theta) \right)
% % \end{equation}

% % Noting that each term in the sum is the negative quantum cross entropy, we can use the result that $\text{tr}(\rho \log \sigma) \leq \log\text{tr}(\rho \sigma)$ \citep{shangnan2021quantum} and write:

% % \begin{equation}
% % \begin{split}
% %     \log P({\bf X}; \theta) &= \sum_{i=1}^D \log \text{tr}\left( \Pi_i \mathcal{E}(\rho_Z^\theta) \right) \\
% %     &\geq \sum_{i=1}^D  \text{tr}\left( \Pi_i  \log \mathcal{E}(\rho_Z^\theta) \right)
% % \end{split}
% % \end{equation}

% \section{Algorithm and Computation}

% Here, we discuss some assumptions  and computational tricks we use to implement scalable IBU for measurement error mitigation.

% \paragraph{Fast Implementation} First, we show how to vectorize the IBU update rule given in Equation \ref{eq:ibu} enabling fast parallel computation on GPUs. Let $\vec{c} \in \mathds{R}^{2^N}$ with $c_i = \frac{n(X_i)}D$, ${\theta_t} \in \mathds{R}^{2^N}$ with $({\theta_t})_i = P_{\theta_t}(Z_i)$, and response matrix $R \in \mathds{R}^{2^N \times 2^N}$ where $R_{ij} = P(X_i | Z_j)$. Then, the IBU update rule can equivalently be written as:


% \begin{equation}\label{eq:ibu}
% \begin{split}
%     \left(\theta_{t+1}\right)_k &= \sum_{i=1}^{2^N} c_i  \cdot \frac{R_i \odot {\theta_t}}{R_i {\theta_t}} \\
%     &= \left(\vec{c}^T \cdot  \text{diag}\left(\frac1{R{\theta_t}}\right) \cdot R \cdot \text{diag}({\theta_t})\right)^T \\
%     &= {\theta_t} \odot \left(R^T\left(\vec{c} \oslash R{\theta_t}\right)\right)
% \end{split}
% \end{equation}

% Here, $\odot$ is element-wise multiplication and $\oslash$ is elementwise division. This expression fully vectorizes the IBU update rule by writing it solely in terms of elementwise products and matrix products. Further, notice that we do not explicitly compute the posterior $P(Z|X)$ as in the original derivation as this only increases memory requirements; instead, we optimize the order of operations so only the additional memory for storing $\theta_{t+1}$ is needed. 


% \paragraph{Tensor Product Structure of Noise Model} Despite the efficient update scheme above, the memory requirements are still quite unfavorable. As previously discussed, the first big memory bottleneck is that the response matrix $R$ grows exponentially in the number of qubits: it is $2^N \times 2^N$. To get around this issue, we can assume that this matrix has a tensor product decomposition into single-qubit conditional probability tables \citep{maciejewskiMitigationReadoutNoise2020, bravyiMitigatingMeasurementErrors2021, nation2021scalable}


% The conditional probability table of the noise model has a tensor decomposition into single-qubit conditional probability tables, i.e., $R = R_1 \otimes R_2 \otimes \ldots \otimes R_N$.


% With this tensor product structure on $R$, we now have $4N$ parameters to represent $R$, as opposed to the original $4^N$ parameters. This structure also allows matrix product $R\vec{x}$ to be computed very quickly using only matrix products and reshapes \citep{fackler2019algorithm} without any additional memory requirement.

% This is the simplest structure we can impose on ${\bf A}$ to obtain tractability. However, this can be relaxed into other tensor network decompositions of ${\bf A}$ as well (such as matrix product states (MPS)); the primary goal is to avoid the exponential scaling in parameters.


% \paragraph{Subspace Reduction for Tractability}

% While we managed the exponential scaling of ${\bf A}$ with a tensor product decomposition, the parameters of the latent distribution $\theta \in \mathds{R}^{2^N}$ also scale exponentially in the number of qubits. To manage this, we can use the subspace reduction approach of \citep{nation2021scalable}: instead of maintaining and updating a vector of probabilities over $2^N$ bitstrings, we only maintain and update $M$-dimensional vector over select bitstrings. Specifically, we pre-select $M$-bitstrings (e.g. to be all those bitstrings within Hamming distance $d$ from any bitstring in our dataset), and initialize $\theta_t$ with non-zero values in the entries corresponding to those $M$ bitstrings. All other entries are taken to be zero. Under such an initialization $\theta_0$, the IBU update rule will guarantee that all entries that started off zero remain zero. Thus, we can ignore those entries and track only the $M \times 1$ sub-vector corresponding to non-zero entries.

% Under this subspace reduction trick, we can no longer easily leverage the Kronecker product structure of ${\bf A}$ to easily compute ${\bf A}\vec{x}$ for any $\vec{x}$. Instead, we must construct a reduced matrix $\tilde{\bf A}$ whose rows and columns correspond to the $M$ selected bitstrings. Unlike \citep{nation2021scalable}, we are not solving a least squares problem, so matrix-free methods like GMRES will not be of help; we really need to construct the reduced matrix $\tilde{\bf A}$. Even if the matrix does not grow exponentially with the number of qubits, it may still be prohibitively large to store in memory.

% Our computational solution to this problem is to use the JAX library's built-in vectorization feature to implement a just-in-time matrix multiplication: each row of the matrix is computed, dotted with $\vec{x}$, and discarded -- all in parallel on a GPU. Although we incur the cost of repeatedly computing $\tilde{\bf A}$, we trade this off against memory constraints in storing ${\bf A}$. Should memory constraints not be the dominant concern, we can simply cache $\tilde{\bf A}$ after the first computation.

% \begin{algorithm}[h]
% \SetAlgorithmName{Algorithm}{}
% \DontPrintSemicolon
% \KwIn{$\vec{c}$ (Vector of normalized counts for each bitstring), $\{{\bf A}_i\}_{i=1}^N$ ($N$ single-qubit error probabilities), $\theta_0$ (initial guess of MEM distribution)} 
% \KwOut{$\theta_T$ (MEM distribution) } 

% % Assign (expert, target, source) roles as follows: $(A, B, C)$, $(B, C, A)$, $(C, A, B)$.\\
% \While{not converged}{

% Compute $\vec{x}_1 = ({A_1} \otimes A_2 \otimes \ldots \otimes A_N){\theta_t}$ using \citep{fackler2019algorithm} if no subspace reduction, or using JIT-compiled vectorized JAX code if using subspace reduction \\

% Compute $\vec{x}_2 = \vec{c} \oslash \vec{x}_1$ \\

% Compute $\vec{x}_3 = {\bf A}^T \vec{x}_2$ using \citep{fackler2019algorithm} if no subspace reduction, or using JIT-compiled vectorized JAX code if using subspace reduction \\

% Compute $\theta_{t+1} = \theta_t \odot \vec{x}_3$.

% }
% Return $\theta_T$
% \caption{Scalable IBU}
% \end{algorithm}

% % \section{IBU vs. Least Squares}

% % \subsection{Negative Probabilities}

% \section{Demonstrations}

% We demonstrate our method on three datasets. First, we consider preparation of the GHZ state, $| \text{GHZ}(n) \rangle = \frac{| 0 \rangle^{\otimes n} + | 1 \rangle^{\otimes n} }{ \sqrt{2} }$ on a simulator. The simulator only accounts of measurement errors, which are modeled after one of the IBMQ QCs, ibmq\_cairo. We sample the probability distributions over 1000 times and show that this finite sampling, without the presence of any decoherence or error in learning the response matrix $M$, is enough to degrade the performance of QREM methods. We also test how existence of negative probabilities in the mitigated quasi-probability distributions is affected by finite sampling errors.

% We then generate GHZ states for various $n$ values on the 127-qubit ibmq\_washington. To reduce circuit-depth, the entangling operation is implemented by parallelizing the two-qubit operations as much as is allowed by the device architecture (please see the appendix for details). Even though we generated GHZ state for up to $n=127$, the probability distribution is identical to a random distribution at $n=82$ so we use that as an upper limit for our analysis. The experiments here were repeated for 100000 shots and the results were bootstrapped using the observed counts. 



% Lastly, we test our method (and M3) on the Bernstein-Vazirani algorithm. This data, which was originally collected by Ref.~\cite{pokharelDemonstrationAlgorithmicQuantum2022}, was taken from a publicly available repository. This is an oracular algorithm where a hidden bitstring $b \in \{ 0,1 \}^n $ is known the oracle, but when inquired with a known bitstring $x \in \{ 0,1 \}^n $ the oracle reveals $x \oplus b$, here $\oplus$ is bit-wise addition. Classically, this algorithm requires $O(n)$ queries but the BV algorithm solves this problem with $O(1)$ query. Theoretically, regardless of the problem size or the hidden bitstring, the success probability for BV is always one. This expectation is violated for a real quantum computer which is subject to decoherence.  The original reference compared how the average success probability changes as a function of problem size and also claimed the quantum strategy can outperform the classical strategy despite a decay in the success probability with increasing problem size. 




% \section{Results}

% \subsection{Bernstein-Vazirani algorithm}

% \begin{figure}[t]
% \centering
% \vspace{-5mm}
%     \begin{displaymath}
% \large
% \Qcircuit @C=1em @R=0.9em @!R {
%  & & &  \mbox{\ \ \ \ \ \ \ Oracle} &  &  \\
% \lstick{| 0 \rangle} & \gate{H} & \ctrl{5} & \qw & \qw & \qw & \gate{H} & \meter  \\
% \lstick{| 0 \rangle} & \gate{H} & \qw & \ctrl{4} & \qw & \qw & \gate{H} & \meter  \\
% & \vdots &  & & & & \vdots & \vdots  \\
% \lstick{| 0 \rangle}  & \gate{H} & \qw & \qw & \ctrl{2} & \qw & \gate{H} & \meter  \\
% \lstick{| 0 \rangle} & \gate{H} & \qw & \qw & \qw & \ctrl{1} & \gate{H} & \meter  \\
% \lstick{| 1 \rangle}  & \gate{H}  & \targ & \targ & \targ & \targ & \gate{H} & \meter \gategroup{2}{3}{7}{6}{0.6em}{-}
% }
%     \end{displaymath}
% \caption{Circuit diagram for the Bernstein-Vazirani algorithm with the hidden bitstring $b=1\dots1$.
% \label{fig:bv_circuit}}

% \end{figure}

% As this problem employs up to 27-qubits on a bona-fide quantum algorithm, we explored whether measurement error mitigation can improve this success probability. \cref{fig:bv} shows that a statistically significant improvement in the success probability is possible due to measurement error mitigation. The effect of MEM gets more pronounced as the problem size increases. This is to be expected as more qubits mean more measurement errors. Additionally, as the decoherence degrades algorithmic performance correction of systematic errors has relatively large role to play. In terms of the success probability, IBU's performance is about equal to or better than state-of-the-art M3 method. While success probability metric is unaffected by negative probabilities, these probabilities are present in the quasi-probability solutions provided by M3. In terms of runtime, the full IBU is noticeably faster than M3 while the reduced version is slightly slower. Recall that full IBU is faster it has a larger memory requirement and reduced IBU is less memory intensive but can be somewhat lower. For a smaller number of qubits relying on full IBU is reasonable, but the memory constraints become the bottleneck for larger problem sizes. 

% We are not making any quantum speedup claims; hybrid issue; Any classical MEM is hybrid; Making claim such after classical MEM is fraught.


% % \begin{figure*}
% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=0.6\textwidth]{bv_figs/bv_logpbar1_aristotle.png}
% %     \caption{Average Success Probability for BV on a log-linear scale.  \bbk{Increase the marker size, unfold the labels, bold the legends.}}
% %     \label{fig:my_label}
% % \end{subfigure}

% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=0.4\textwidth]{bv_figs/bv_tnp_aristotle.png}
% %     \caption{The total `negative probability' mass of the measurement-error corrected result}
% %     \label{fig:my_label}
% % \end{subfigure}


% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=0.4\textwidth]{bv_figs/bv_rt_aristotle.png}
% %     \caption{The total run-time of various mitigation methods on our machine.}
% %     \label{fig:my_label}
% % \end{subfigure}
% % \caption{BV algorithm was implemented on the 27-qubit IBMQ Cairo. For the top figure we restrict ourselves to larger problem sizes as the mitigated results are identical to the unmitigated ones.  The data was taken from a publicly available source.BV algorithm was implemented on the 27-qubit IBMQ Cairo. The data was taken from a publicly available source.}
% % \end{figure*}

% \begin{figure*}
%     \centering
%     \begin{minipage}{0.6\linewidth}
%             \begin{subfigure}{}
%                 \includegraphics[trim = 50 0 100 100, clip,width=\textwidth]{bv_figs/bv_logpbar1_aristotle.png}
%             \end{subfigure}
%         \end{minipage}
%     \begin{minipage}{0.38\linewidth}
%         \begin{subfigure}{}
%             \includegraphics[trim = 0 70 100 0, clip, width=\textwidth]{bv_figs/bv_tnp_aristotle.png}
%             \label{fig:weather_filter1}
%         \end{subfigure} \\
%         \vspace{-11mm}
%         \begin{subfigure}{}
%             \includegraphics[trim = 0 0 100 70, clip, width=\textwidth]{bv_figs/bv_rt_aristotle.png}
%             \label{fig:weather_filter2}
%         \end{subfigure} 
%     \end{minipage}
%     \caption{\emph{Bernstein-Vazirani Algorithm:} BV algorithm was implemented on the 27-qubit IBMQ Cairo. For the top figure we restrict ourselves to larger problem sizes as the mitigated results are identical to the unmitigated ones.  The data was taken from a publicly available source.BV algorithm was implemented on the 27-qubit IBMQ Cairo. The data was taken from a publicly available source.  \label{fig:bv}}
% \end{figure*}




% \subsection{Generating GHZ states}

% GHZ states are prepared by entangling $n$ qubits. This means that as long as there is a single connection allowing for a multi-qubit entangling operation like CNOT, it is possible to create a GHZ state linearly increasing in circuit depth. Decoherence is introduced both by multi-qubit operations (which are noisy), and by the total circuit duration. In order to restrict circuit duration, we apply these CNOTs in parallelized manner. Starting from the most connected qubit (the qubit with the greatest number of connections/edges to neighouring qubits) in a superposition state $|+\rangle$, we use CNOT gates to entangle every additional qubit with breadth-first search. In effect, this amounts to prioritizing the distance $1$ neighbours to entangle, followed by the distance $2$ neighbours, and so on. This strategy limits circuit depth and minimizes decoherence. We give a visualization in \bbk{figure oslo}.

% \begin{figure}
% \includegraphics[trim = 70 70 70 70,clip,width=0.7\columnwidth]{ibmq_jakarta_gate_map.pdf}
%  \begin{displaymath}
%  \large
%     \Qcircuit @C=1.0em @R=0.2em @!R { \\
%  \lstick{{q}_{0}} & \qw & \qw & \targ & \qw & \qw & \qw & \meter\\
% \lstick{{q}_{1}} & \gate{\mathrm{H}} & \ctrl{2} & \ctrl{-1} & \ctrl{1} & \qw & \qw & \meter\\
% \lstick{{q}_{2}} & \qw & \qw & \qw & \targ & \qw & \qw & \meter\\
% \lstick{{q}_{3}} & \qw & \targ & \ctrl{2} & \qw & \qw & \qw & \meter\\
% \lstick{{q}_{4}} & \qw & \qw & \qw & \targ & \qw & \qw & \meter\\
% \lstick{{q}_{5}} & \qw & \qw & \targ & \ctrl{-1} & \ctrl{1} & \qw & \meter\\
% \lstick{{q}_{6}} & \qw & \qw & \qw & \qw & \targ & \qw & \meter
% 	 	}
%  \end{displaymath}
%     \caption{Example of GHZ generation circuit: Given a 7-qubit architecture (top), the GHZ generation circuit is created by first identifying an vertex with maximum possible degree (q1) and then performing a breadth-first and performing CNOTs accordingly to create a fully-entangled state. For our experiments, we generated GHZ on an 127-qubit device, but here we demonstrate the scheme on a 7-qubit device for simplicity.}
%     \label{fig:my_label}
% \end{figure}

% % \subsubsection{Simulation}




% % \begin{figure}[htpb!]
% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=\textwidth/2]{ghz_sim_figs/ghz_sim_errors0.png}
% %     \caption{\emph{(GHZ Sim)} Error in $\ell_1$ norm between the error mitigated result and the GHZ state in the computational basis \bbk{Normalize (1- 0.5 l1)}}
% %     \label{fig:my_label}
% % \end{subfigure}

% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=\textwidth/2]{ghz_sim_figs/ghz_sim_neg.png}
% %     \caption{\emph{(GHZ Sim)} The total `negative probability' mass of the measurement-error corrected result, by mitigation method. }
% %     \label{fig:my_label}
% % \end{subfigure}


% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=\textwidth/2]{ghz_sim_figs/ghz_sim_rt.png}
% %     \caption{\emph{(GHZ Sim)} The run-time of various mitigation methods on our machine.}
% %     \label{fig:my_label}
% %     \end{subfigure}
% % \end{figure}



% \begin{figure*}
%     \centering
%     \begin{minipage}{0.6\linewidth}
%             \begin{subfigure}{}
%                 \includegraphics[trim = 50 0 100 100, clip,width=\textwidth]{ghz_sim_figs/ghz_sim_errors0.png}
%             \end{subfigure}
%         \end{minipage}
%     \begin{minipage}{0.38\linewidth}
%         \begin{subfigure}{}
%             \includegraphics[trim = 0 70 100 0, clip,width=\textwidth]{ghz_sim_figs/ghz_sim_neg.png}
%         \end{subfigure} \\
%                 \vspace{-7.6mm}
%         \begin{subfigure}{}
%             \includegraphics[trim = 0 0 100 70, clip,width=\textwidth]{ghz_sim_figs/ghz_sim_rt.png}
%         \end{subfigure} 
%     \end{minipage}
%     \caption{\emph{Simulated GHZ state preparation:} State Preparation of GHZ state was done in presence of measurement errors. All circuit-based decoherence was disabled. Even in this idealized simulation, finite sampling error is sufficient for existence of negative probability in the mitigated quasi-probability distributions. Moreover, $\ell_1$-error and total negative probability are both shown to grow with the number of qubits.  }
% \end{figure*}


% \subsubsection{IBM Washington}

% 1) Sell IBU: reduced l1 errors, increased 0s and 1s probability, 

% \paragraph{comments on error} We use l1 error and normalize it for convenience. This is not a perfect metric as we only have measurements in the $Z$ basis. 
% Under our normalized l1 error metric we are able to correct measurement errors and 

% \paragraph{comments on run time} linear in per-iteration run time is linear in the number of

% \paragraph{comments on negative probabilities} At these large size you get significant negative probabilities; also comment about downsampled error

% We have also seen this in simulated results; 

% Substantial negative probabilities in M3; (cannot just project as it zeros bitstrings)




% % \begin{figure}

% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=\textwidth/2]{ghz_wash_figs/ghz_ibm_errors0.png}
% %     \caption{\emph{(GHZ on IBM Washington)} $\frac12 (\ell_1 \text{ error})$ between the error mitigated result and the GHZ state. The theoretical minimum should be 0, and M3 falls under this because of `negative probabilities' in the error mitigated result.}
% %     \label{fig:my_label}
% % \end{subfigure}

% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=\textwidth/2]{ghz_wash_figs/ghz_ibm_neg.png}
% %     \caption{\emph{(GHZ on IBM Washington)} The total `negative probability' mass of the measurement-error corrected result, by mitigation method.}
% %     \label{fig:my_label}
% % \end{subfigure}


% % \begin{subfigure}
% %     \centering
% %     \includegraphics[width=\textwidth/2]{ghz_wash_figs/ghz_ibm_rt.png}
% %     \caption{\emph{(GHZ on IBM Washington)} The run-time of various mitigation methods on our machine.}
% %     \label{fig:my_label}
% % \end{subfigure}
% % \end{figure}


% \begin{figure*}
%     \centering
%     \begin{minipage}{0.6\linewidth}
%             \begin{subfigure}{}
%                 \includegraphics[trim = 50 0 100 100, clip,width=\textwidth]{ghz_wash_figs/ghz_ibm_errors0.png}
%             \end{subfigure}
%         \end{minipage}
%     \begin{minipage}{0.38\linewidth}
%         \begin{subfigure}{}
%             \includegraphics[trim = 0 70 100 0, clip,width=\textwidth]{ghz_wash_figs/ghz_ibm_neg.png}
%         \end{subfigure} \\
%                 \vspace{-7.3mm}
%         \begin{subfigure}{}
%             \includegraphics[trim = 0 0 100 70, clip,width=\textwidth]{ghz_wash_figs/ghz_ibm_rt.png}
%         \end{subfigure} 
%     \end{minipage}
%     \caption{\emph{GHZ state preparation on 127-qubit IBMQ Washington:} We attempted to create GHZ states on up to 127-qubits. However, the probability distribution was indistinguishable from a random distribution beyond 82-qubits. At all problem sizes, IBU returns a higher value from the performance metric $1- \frac12 (\ell_1 \text{ error})$. The theoretical minimum should be 0, but M3 gives negative values due to the presence of negative probabilities in the quasi-probability distribution. Runtime for IBU is much longer than for M3 but plateaus at around 80 qubits. Note that the runtime scales not with the number of qubits but the number of shots and therefore both M3 and IBU are scalable to higher number of qubits.  }
% \end{figure*}

% \section{Discussion and Conclusion}



% \newpage 

% \bibliography{biblio.bib, mem.bib}


% \pagebreak

% \section{Appendix}

% \section{MAP IBU}

% Here we suggest a simple Bayesian extension of IBU: allowing us to impose a prior on the parameters $P(\theta)$ and identifying the Maximum a posteriori (MAP) estimate of the parameters $P(\theta | {\bf X})$. We begin by observing that:

% \begin{equation}
%     \begin{split}
%         \log P(\theta | {\bf X}) &= \log P({\bf X} | \theta) + \log P(\theta) - \log P({\bf X})
%     \end{split}
% \end{equation}

% Since we wish to find the choice of $\theta$ at which the posterior is maximized, we ignore $\log P({\bf X})$. Further, by Equation \ref{eq:bound}, we know that $\log P({\bf X} | \theta) \geq \hat{\ell}(\theta|\theta_t; {\bf X})$. Similar to the previous approach, instead of directly maximizing the posterior, we seek to maximize the lower-bound:

% \begin{equation}
%     \theta_{t+1} = \underset{\theta}{\text{arg max } } \hat{\ell}(\theta|\theta_t; {\bf X}) + \log P(\theta)
% \end{equation}

% For our purposes, we assume that the prior over parameters is specified as a Dirichlet distribution with parameter $\boldsymbol{\alpha} \in \mathds{R}^{2^N}$, and let $K= \sum_j \alpha_j$. This is a natural choice as Dirichlet distributions are the conjugate prior for multinomial distribution. Thus, $P(\theta) = \frac1{B(\boldsymbol{\alpha})} \prod_{j=1}^{2^N} \theta_j^{\alpha_j - 1}$ where $B(\cdot)$ is the beta function.

% \begin{equation}
%     \begin{split}
%         &\phantom{=} \frac{\partial }{ \partial \theta_k} \left( \hat{\ell}(\theta|\theta_t; {\bf X}) + \log P(\theta) + \lambda \left(1 - \sum_{j=1}^{2^N} \theta_j \right)\right) \\
%         &= \left(\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)\frac1{\theta_k} - \lambda + \frac{\partial }{ \partial \theta_k} \left( \log P(\theta)\right) \\
%         &= \left(\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)\frac1{\theta_k} - \lambda + \frac{\partial }{ \partial \theta_k} \log \left(  \frac1{B(\boldsymbol{\alpha})} \prod_{j=1}^{2^N} \theta_j^{\alpha_j - 1}\right) \\
%         &= \left(\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)\frac1{\theta_k} - \lambda + \frac{\partial }{ \partial \theta_k} \sum_{j=1}^{2^N} ({\alpha_j - 1}) \log \left(   \theta_j\right) \\
%         &= \left(\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)\frac1{\theta_k} - \lambda + \frac{\alpha_k - 1}{\theta_k}
%     \end{split}
% \end{equation}

% Setting this to zero, we get $\theta_k = \frac1{\lambda}\left((\alpha_k - 1) + \sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)$, and by the requirement that 

% \begin{equation}
% \begin{split}
%     &\phantom{=} \sum_{k=1}^{2^N} \theta_k = 1 \\
%     &\Rightarrow \sum_{k=1}^{2^N} \frac1{\lambda}\left((\alpha_k - 1) +\sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right) = 1 \\
%     &\Rightarrow \lambda = \sum_{k=1}^{2^N} (\alpha_k - 1) +  \sum_{i=1}^D \sum_k P_{\theta_t}(Z_k|X_i) \\
%     &\Rightarrow \lambda = D + K - 2^N
% \end{split}
% \end{equation}

% Substituting this back in, we get our update rule for each element $\theta_k$ of $\theta$ that locally maximizes the log-likelihood given an initial guess $\theta_t$:

% \begin{equation}
%     \left(\theta_{t+1}\right)_k =  \frac1{D + K - 2^N}\left((\alpha_k - 1) + \sum_{i=1}^D P_{\theta_t}(Z_k|X_i) \right)
% \end{equation}

% As before, we can rewrite the sum with  counts $n(X_i)$ and use Bayes' rule to arrive at the update rule:

% \begin{equation}\label{eq:mapibu}
%     \left(\theta_{t+1}\right)_k = \frac{\alpha_k - 1}{D+K-2^N} + \sum_{i=1}^{2^N} \frac{n(X_i)}{D + K - 2^N}  \cdot \frac{P(X_i | Z_k) P_{\theta_t}(Z_k)}{\sum_i P(X_i | Z_k) P_{\theta_t}(Z_k)}
% \end{equation}

% If we impose a uniform prior by setting $\alpha_k = 1$ for all $k$, then Equation \ref{eq:mapibu} clearly reduces to standard IBU as in Equation \ref{eq:ibu}. When using non-uniform priors, MAP-IBU prevents the parameters from updating too far away from the specified prior.


% \subsection{Bernstein-Vazirani}
% \begin{figure*}[htpb!]
%     \centering
%     \includegraphics[width=\textwidth]{bv_figs/bv_logpbar_aristotle.png}
%     \caption{\emph{(Bernstein-Vazirani} The average success probability for each problem size, both with and without dynamical decoupling (DD). The classical baseline is shown by the dotted line.}
%     \label{fig:my_label}
% \end{figure*}


% \subsection{GHZ Sim}
% \begin{figure*}[htpb!]
%     \centering
%     \includegraphics[width=\textwidth]{ghz_sim_figs/ghz_sim_errors2.png}
%     \caption{\emph{(GHZ Sim)} Error in $\ell_1$ and $\ell_\infty$ norms between mitigated results and the GHZ state in the computational basis}
%     \label{fig:my_label}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{ghz_sim_figs/ghz_sim_zo2.png}
%     \caption{\emph{(GHZ Sim)} The probability assigned to the solution bitstrings (all 0s [left] and all 1s [right]).}
%     \label{fig:my_label}
% \end{figure*}


% \subsection{IBM Washington}

% \begin{figure*}[htpb!]
%     \centering
%     \includegraphics[width=\textwidth]{ghz_wash_figs/ghz_ibm_ev2.png}
%     \caption{\emph{(GHZ on IBM Washington)} Expectation Value of the $Z$-operator on even-numbered qubit systems. The GHZ state should give an expectation of 1.}
%     \label{fig:my_label}
% \end{figure*}



% \begin{figure*}[htpb!]
%     \centering
%     \includegraphics[scale=0.25]{ghz_wash_figs/ghz_ibm_errors2.png}
%     \caption{\emph{(GHZ on IBM Washington)} Error in $\ell_1$ and $\ell_\infty$ norms of the mitigatied distribution with respect to GHZ state in computational basis.}
%     \label{fig:my_label}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[scale=0.25]{ghz_wash_figs/ghz_ibm_zo2.png}
%     \caption{\emph{(GHZ on IBM Washington)} Probability of All 0s (left) and All 1s (right)}
%     \label{fig:my_label}
% \end{figure*}



% \begin{figure}{}
%     \includegraphics[trim = 0 0 100 70, clip, width=\textwidth]{ghz_wash_figs/ghz_ibm_rt2.png}
%     \label{fig:ibmrt2}
% \end{figure} 
        
        
% \section{Device Specifications}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{|l|c|c|c|c|c|c|}
%     \hline
%         ~ & \multicolumn{2}{c}{Montreal}  & & \multicolumn{2}{c}{Washington} &  \\ \hline
%         ~ & Min & Mean & Max & Min & Mean & Max \\ \hline
%         $T_1$ ($\mu$s) & 57.57 & 113.2 & 187.1 & 40.43 & 101.98 & 247.7 \\ \hline
%         $T_2$ ($\mu$s) & 22.58 & 99.72 & 198.71 & 2.61 & 94.29 & 259.39\\ \hline
%         1QG Error  (\%) & 0.02 & 0.04 & 0.15 & 0.02 & 0.08 & 1.09 \\ \hline
%         2QG Error  (\%) & 0.57 & 1.35 & 6.09 &  0.53 & 4.79 & 100.   \\ \hline
%         1QG Duration ($\mu$s) & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 \\ \hline
%         2QG Duration ($\mu$s) & 0.27 & 0.43 & 0.63 & 0.27 & 0.55 & 1.34 \\ \hline
%         RO Error (\%) & 0.79 & 2.59 & 10.66 & 0.23  & 3.51 & 38.49 \\ \hline
%         RO Duration  ($\mu$s) & 5.2 & 5.2 & 5.2 & 0.86 & 0.86 & 0.86 \\ \hline
%     \end{tabular}
% \caption{Device specifications for Montreal and Washington. 1QG and 2QG denote 1-qubit gate and 2-qubit gate, respectively. RO denotes readout.}
% \label{tab:device}
% \end{table}

% \begin{figure*}{htpb}
%     \includegraphics[ width=\textwidth]{montreal_backend_map.png}
%     \label{fig:montreal-connectivity}
% \end{figure*} 

% \begin{figure*}{htpb}
%     \includegraphics[ width=\textwidth]{ibm_washington.png}
%     \label{fig:montreal-connectivity}
% \end{figure*} 

% \end{document}
